When did you become so smart, oh wise one?! Sarcasm Explanation in Multi-modal Multi-party Dialogues

Indirect speech such as sarcasm achieves a constellation of discourse goals in human communication. While the indirectness of figurative language warrants speakers to achieve certain pragmatic goals, it is challenging for AI agents to comprehend such idiosyncrasies of human communication. Though sarcasm identification has been a well-explored topic in dialogue analysis, for conversational systems to truly grasp a conversation's innate meaning and generate appropriate responses, simply detecting sarcasm is not enough; it is vital to explain its underlying sarcastic connotation to capture its true essence. In this work, we study the discourse structure of sarcastic conversations and propose a novel task - Sarcasm Explanation in Dialogue (SED). Set in a multimodal and code-mixed setting, the task aims to generate natural language explanations of satirical conversations. To this end, we curate WITS, a new dataset to support our task. We propose MAF (Modality Aware Fusion), a multimodal context-aware attention and global information fusion module to capture multimodality and use it to benchmark WITS. The proposed attention module surpasses the traditional multimodal fusion baselines and reports the best performance on almost all metrics. Lastly, we carry out detailed analyses both quantitatively and qualitatively.

==> Tables/human_eval-eg.tex <==
\begin{table*}[ht]
\centering
\subfloat[Incoherant dialogue]{
\label{tab:coherence}
\resizebox{0.33\textwidth}{!}{%
\begin{tabular}{p{4em}p{20em}}
\multicolumn{2}{c}{\includegraphics[\textwidth]{Figures/human_eval_eg_2_1.pdf}} \\ \hline
\multicolumn{2}{}{\begin{tabular}[c]{@{}p{25em}@{}}{ROSESH:} What nonsense? Mujhe kon hunter marega? \textit{\color{blue}What nonsense? Who will beat me with a hunter?}\\{INDRAVARDHAN:} Me, me marunga. Kyunki 51 saal baad Maya to mar chuki hogi. Me kisi tarah zinda reh lunga or kahunga ki `le mar jhadhu, mar, mar jhadhu, mar mar' \textit{\color{blue}Me. I will beat you. Because after 51 years, Maya would be dead. I'll somehow stay alive and will say `sweep here. sweep here, sweep sweep'}\end{tabular}} \\ \hline
\rowcolor{LightGreen}\bf Ground Truth & Maya Monisha ko tana marti hai safai ka dhyan na rakhne ke liye \textit{\color{blue}Maya taunts Monisha for not keeping a check of cleanliness}\\ 
\rowcolor{LightGreen} & \\
 & \\
\bf Predicted & Maya implies ki Monisha bohot ghar mein bahar nahi kar sakati \textit{\color{blue} Maya implies that Monisha very home outside cannot do}\\
\hline
\end{tabular}
}
}
\subfloat[Explanation related to dialogue but not with sarcasm]{
\label{tab:context}
\resizebox{0.33\textwidth}{!}{%
\begin{tabular}{p{4em}p{20em}} 
\multicolumn{2}{c}{\includegraphics[\textwidth]{Figures/human_eval_eg_2_2.pdf}} \\ \hline
\multicolumn{2}{}{\begin{tabular}[c]{@{}p{24em}@{}}MAYA: Hi baby! \textit{\color{blue}Hi baby!}\\ROSESH: Mai bhi chalu, aap ke saath, Sudhanshu ke island par? \textit{\color{blue}Can I also go, with you, to Sudhanshu's island?}\\MAYA: Oh sweetie... Mai apane saath aisi koi bhi cheez nahi le jana chaahati jo mujhe apani pichli zindagi ki yaad dilaye... \textit{\color{blue}Oh sweetie... I don't want to take anything with me that reminds me of my past life...}\end{tabular}} \\
 & \\
\hline
\rowcolor{LightGreen}\bf Ground Truth & Maya implies ki vo Rosesh ko apane saath Sudhanshu ke island par nahi je jaana chaahati \textit{\color{blue}Maya implies that she does not want to take Rosesh with her to Sudhanshu's island} \\ 
 & \\
\bf Predicted & Maya Rosesh ko apani pichaali zinday se compare hone par taunt maarti hai \textit{\color{blue}Maya taunts Rosesh by comparing him with her past life}\\
\hline
\end{tabular}
}
}
\subfloat[Explanation related to sarcasm]{
\label{tab:sarcasm}
\resizebox{0.33\textwidth}{!}{%
\begin{tabular}{p{4em}p{20em}}
\multicolumn{2}{c}{\includegraphics[\textwidth]{Figures/human_eval_eg_2_3.pdf}} \\ \hline
\multicolumn{2}{}{\begin{tabular}[c]{@{}p{24em}@{}}MONISHA: Ladki ka naam Ajanta Kyon Rakha? \textit{\color{blue}Why did they named the girl Ajanta?}\\INDRAVARDHAN: Kyunki uski maa ajanta caves dekh rahi thi Jab vo Paida Hui haha. \textit{\color{blue}Because her mother must be watching the Ajanta caves when she was born haha.}\end{tabular}}\\
 & \\
 & \\ 
 & \\\hline
\rowcolor{LightGreen} \bf Ground Truth & Indravadan ajanta ke naam ka mazak udata hai \textit{\color{blue}Indravardhan makes fun of Ajanta's name} \\
\rowcolor{LightGreen}& \\
\rowcolor{LightGreen}& \\
 & \\
\bf Predicted & Indravadan ajanta ke naam ka mazak udata hai \textit{\color{blue}Indravardhan makes fun of Ajanta's name}\\
 & \\ \hline
\end{tabular}
}
}
\caption{Examples of factors considered for human evaluation- coherence, related to dialogue, and related to sarcasm.}
\end{table*}

==> Tables/human_eval-multimodality.tex <==
\begin{table}[h!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
 & \textbf{Coherency} & \textbf{Related to dialogue} & \textbf{Related to sarcasm} \\ \hline
\textbf{BART-T} &  &  &  \\ \hline
\textbf{AVII-BART-TA} &  &  &  \\ \hline
\textbf{AVII-BART-TV} &  &  &  \\ \hline
\textbf{AVII-BART-TAV} &  &  &  \\ \hline
\end{tabular}%
}
\caption{Human evaluation multimodality}
\label{tab:human_eval_multimodality}
\end{table}

==> Tables/results-fusion-english.tex <==
\begin{table*}[]
\centering
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{} & \textbf{Rouge-1} & \textbf{Rouge-2} & \textbf{Rouge-L} & \textbf{BLEU-1} & \textbf{BLEU-2} & \textbf{BLEU-3} & \textbf{BLEU-4} & \textbf{METEOR} \\ \hline
\textbf{Concat-TAV} &  &  &  &  &  &  &  &  \\ \hline
\textbf{SelfAttention-TAV} &  &  &  &  &  &  &  & \\ \hline
% \textbf{Fusion1-TAV} &  &  &  &  &  &  &  & \\ \hline
\textbf{AVII-TAV} & \bf 43.49 & \bf 20.69 & \bf 40.39 & 34.14 & 20.51 & 13.68 & 9.38 & 32.1 \\ \hline
\end{tabular}%
}
\caption{Fusion-English}
\label{tab:fusion-english}
\end{table*}

==> Tables/results-fusion.tex <==
\begin{table}[h!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|ll|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{2}{|l|}{} & R1 & R2 & RL & B1 & B2 & B3 & B4 & METEOR \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{Code-mixed}} & Concat-TAV &  &  &  &  &  &  &  &  \\ \cline{2-10} 
\multicolumn{1}{|l|}{} & SelfAttention-TAV &  &  &  &  &  &  &  &  \\ \cline{2-10} 
\multicolumn{1}{|l|}{} & AVII-TAV & \bf 43.49 & \bf 20.69 & \bf 40.39 & 34.14 & 20.51 & 13.68 & 9.38 & 32.1 \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{English}} & Concat-TAV &  &  &  &  &  &  &  &  \\ \cline{2-10} 
\multicolumn{1}{|l|}{} & SelfAttention-TAV &  &  &  &  &  &  &  &  \\ \cline{2-10} 
\multicolumn{1}{|l|}{} & AVII-TAV & \bf 43.49 & \bf 20.69 & \bf 40.39 & 34.14 & 20.51 & 13.68 & 9.38 & 32.1 \\ \hline
\end{tabular}%
}
\caption{Fusion}
\label{tab:fusion}
\end{table}

==> Tables/results-multimodality-english.tex <==
\begin{table*}[]
\centering
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{} & \textbf{Rouge-1} & \textbf{Rouge-2} & \textbf{Rouge-L} & \textbf{BLEU-1} & \textbf{BLEU-2} & \textbf{BLEU-3} & \textbf{BLEU-4} & \textbf{METEOR} \\ \hline
\textbf{AVII-TA} & 38.90 & 16.38 & 36.51 & 32.63 & 18.14 & 12.00 & 8.02 & 29.66 \\ \hline
\textbf{AVII-TV} & 42.12 & 19.63 & 40.24 & 36.05 & 21.34 & 14.29 & 10.35 & 33.28 \\ \hline
\textbf{AVII-TAV} & \bf 43.49 & \bf 20.69 & \bf 40.39 & 34.14 & 20.51 & 13.68 & 9.38 & 32.1 \\ \hline
\end{tabular}%
}
\caption{Multimodality-English}
\label{tab:multimodality-english}
\end{table*}

==> Tables/results-multimodality.tex <==
\begin{table*}[ht]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{Model} & \textbf{ROUGE 1} & \textbf{ROUGE 2} & \textbf{ROUGE L} & \textbf{BLEU 1} & \textbf{BLEU 2} & \textbf{BLEU 3} & \textbf{BLEU 4} & \textbf{METEOR} \\ \hline \hline
\textbf{m\modelTA} & 39.02 & 15.90 & 36.83 & 31.26 & 16.94 & 11.54 & 7.72 & 29.05 \\ \hdashline
\textbf{m\modelTV} & 39.47 & 16.78 & 37.38 & 32.44 & 17.91 & 12.02 & 7.36 & 29.74 \\ \hdashline
\textbf{m\modelTAV} & 38.52 & 14.12 & 36.60 & 30.50 & 15.20 & 9.78 & 5.74 & 27.42 \\ \hline
\textbf{\modelTA} & 38.21 & 14.53 & 35.97 & 30.58 & 15.36 & 9.63 & 5.96 & 27.71 \\ \hdashline
\textbf{\modelTV} & 37.48 & 15.38 & 35.64 & 30.28 & 16.89 & 10.33 & 6.55 & 28.24 \\ \hdashline
\textbf{\modelTAV} & \textbf{39.69} & \textbf{17.10} & \textbf{37.37} & \textbf{33.20} & \textbf{18.69} & \textbf{12.37} & \textbf{8.58} & \textbf{30.40} \\ \hline
\end{tabular}%
}
\caption{Experimental results for multimodal fusion in unimodal systems. (AII: Audio Information Infused; VII: Visual Information Infused; AVII: Audio-Visual Information Infused)}
\label{tab:multimodality}
\end{table*}

==> Tables/results-text-only-eng.tex <==
\begin{table}[h!]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{|ll|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{2}{|l|}{} & R1 & R2 & RL & B1 & B2 & B3 & B4 & METEOR \\ \hline
\multicolumn{1}{|l|}{\multirow{5}{*}{Code-mixed}} & RNN & 8.94 & 0.98 & 8.61 & 1.24 & 0.29 & 1.63 & 1.22 & 3.30 \\ \cline{2-10} 
\multicolumn{1}{|l|}{} & Transformer & 3.20 & 0.25 & 3.19 & 0.40 & 0.01 & 1.15 & 8.20 & 1.11 \\ \cline{2-10} 
\multicolumn{1}{|l|}{} & PGN & 23.37 & 4.83 & 17.46 & 17.32 & 6.68 & 1.58 & 0.52 & 23.54 \\ \cline{2-10} 
\multicolumn{1}{|l|}{} & BART & \bf 41.49 & 16.66 & \bf 38.81 & \bf 33.27 & 18.00 & 10.87 & 6.71 & 31.88 \\ \cline{2-10} 
\multicolumn{1}{|l|}{} & mBART & 40.82 & 17.35 & 38.08 & 32.75 & 18.33 & \bf 11.8 & \bf 8.31 & 31.12 \\ \hline
\multicolumn{1}{|l|}{\multirow{5}{*}{English}} & RNN & 8.94 & 0.98 & 8.61 & 1.24 & 0.29 & 1.63 & 1.22 & 3.30 \\ \cline{2-10} 
\multicolumn{1}{|l|}{} & Transformer & 3.20 & 0.25 & 3.19 & 0.40 & 0.01 & 1.15 & 8.20 & 1.11 \\ \cline{2-10} 
\multicolumn{1}{|l|}{} & PGN & 23.37 & 4.83 & 17.46 & 17.32 & 6.68 & 1.58 & 0.52 & 23.54 \\ \cline{2-10} 
\multicolumn{1}{|l|}{} & BART & \bf 41.49 & 16.66 & \bf 38.81 & \bf 33.27 & 18.00 & 10.87 & 6.71 & 31.88 \\ \cline{2-10} 
\multicolumn{1}{|l|}{} & mBART & 40.82 & 17.35 & 38.08 & 32.75 & 18.33 & \bf 11.8 & \bf 8.31 & 31.12 \\ \hline
\end{tabular}%
}
\caption{Multilinguality}
\label{tab:multilinguality}
\end{table}

==> Tables/results-text-only.tex <==
\begin{table*}[h!]
\centering
\resizebox{0.9\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{Model} & \textbf{ROUGE 1} & \textbf{ROUGE 2} & \textbf{ROUGE L} & \textbf{BLEU 1} & \textbf{BLEU 2} & \textbf{BLEU 3} & \textbf{BLEU 4} & \textbf{METEOR} \\ \hline
\textbf{RNN} & 8.94 & 0.98 & 8.61 & 1.24 & 0.29 & 1.63 & 1.22 & 3.30 \\ \hline
\textbf{Transformers} & 3.20 & 0.25 & 3.19 & 0.40 & 0.01 & 1.15 & 8.20 & 1.11 \\ \hline
\textbf{PGN} & 23.37 & 4.83 & 17.46 & 17.32 & 6.68 & 1.58 & 0.52 & 23.54 \\ \hline
\textbf{mBART} & 33.66 & 11.02 & 31.50 & 22.92 & 10.56 & 6.07 & 3.39 & 21.03 \\ \hline
\textbf{BART} & 36.88 & 11.91 & 33.49 & 27.44 & 12.23 & 5.96 & 2.89 & 26.65 \\ \hline \hline
\textbf{BART-AVII-TA} & 38.21 & 14.53 & 35.97 & 30.58 & 15.36 & 9.63 & 5.96 & 27.71 \\ \hline
\textbf{BART-AVII-TV} & 37.48 & 15.38 & 35.64 & 30.28 & 16.89 & 10.33 & 6.55 & 28.24 \\ \hline
\rowcolor{LightGreen}\textbf{BART-AVII-TAV} & \bf 39.69 & \bf 17.10 & \bf 37.37 & \bf 33.20 & \bf 18.69 & \bf 12.37 & \bf 8.58 & \bf 30.40 \\ \hline \hline
\textbf{BART-AVII-TAV-no-gating} & 39.95 & 14.85 & 37.18 & 31.85 & 15.97 & 9.62 & 5.47 & 28.87 \\ \hline \hline
\textbf{BART-Concat-TAV} & 8.64 & 0.36 & 8.02 & 5.54 & 0.43 & 0.06 & 1.34 & 5.02 \\ \hline
\textbf{BART-Attention-TAV} & 36.26 & 12.39 & 34.11 & 29.31 & 13.95 & 7.61 & 4.84 & 26.58 \\ \hline
\end{tabular}%
}
\caption{Multilinguality}
\label{tab:multilinguality}
\end{table*}
